MiniRec: Data-Efficient Reinforcement Learning for LLM-based Recommendation

The integration of reinforcement learning (RL) into large language models (LLMs) has opened new opportunities for recommender systems by eliciting reasoning and improving user preference modeling. However, RL-based LLM recommendation faces significant efficiency challenges, making full-data training costly. Existing data selection methods define sample value based on learnability or representativeness, yet their loss- or gradient-driven or dataset coverage-driven criteria often misalign with RL learning dynamics, resulting in suboptimal performance. To address this, we propose MiniRec, a data selection framework tailored for RL-based LLM recommendation. MiniRec evaluates sample learnability using key RL signals -- rewards -- pruning samples that are too easy (too high reward) or too difficult (consistently low reward). It assesses representativeness by aligning sample gradients with the approximated "ideal" global RL optimization trajectory, selecting samples that mainly drive model updates, and it also enforces diversity to reduce redundancy. Combined with a curriculum learning strategy from easy to hard samples, MiniRec significantly reduces training cost while largely preserving performance. Extensive experiments demonstrate MiniRec's effectiveness, highlighting the importance of reward-aligned, trajectory-informed data selection in RL-based LLM recommendation.

==> sections/app.tex <==
\appendix

\section{Implementation Details}

Algorithm~\ref{alg:minirec} outlines the Subset Selection with Curriculum Scheduling procedure. The algorithm first computes three complementary metrics for each sample—learnability, representativeness, and diversity—to evaluate its contribution to the subset. A greedy selection strategy iteratively constructs a subset that balances informativeness and coverage under a predefined target size. After selection, the chosen subset is partitioned into multiple curriculum stages based on sample difficulty, enabling the model to be trained progressively from easier to harder samples. This curriculum-driven subset optimization enhances both data efficiency and generalization during training.

\begin{algorithm}[t]
  \caption{Subset Selection with Curriculum Scheduling}
  \label{alg:minirec}
  \begin{algorithmic}[1]
  
  \REQUIRE Full dataset $\mathcal{D}$, base model $M$, 
  target subset size $m$, balance weight $\lambda$, 
  number of curriculum groups $K$.
  
  \vspace{0.5em}
  \STATE \textbf{Learnability:} 
  Estimate rewards $\bar{r}(x_i)$, compute $L(x_i)$ (Eq.~\eqref{eq:gaussian}), 
  and normalize to $L_{\text{norm}}(x_i)$ (Eq.~\eqref{eq:l_norm}).
  
  \STATE \textbf{Representativeness:} 
  Compute representativeness score $R_{\text{norm}}(x_i)$ for each sample.
  
  \STATE \textbf{Diversity-driven Greedy Selection:}
  \STATE Initialize $\mathcal{S} \leftarrow \emptyset$.
  \WHILE{$|\mathcal{S}| <$ target size $m$}
    \FORALL{$x_i \in \mathcal{D} \setminus \mathcal{S}$}
      \STATE Compute diversity score $D_{\text{norm}}(x_i \mid \mathcal{S})$
             as minimum distance to samples in $\mathcal{S}$.
      \STATE Compute overall value:
        \[
        V(x_i \mid \mathcal{S}) = D_{\text{norm}}(x_i \mid \mathcal{S})
        \cdot \big( L_{\text{norm}}(x_i) + \lambda R(x_i) \big).
        \]
    \ENDFOR
    \STATE Select $x^* = \arg\max_{x_i} V(x_i \mid \mathcal{S})$.
    \STATE Update $\mathcal{S} \leftarrow \mathcal{S} \cup \{x^*\}$.
  \ENDWHILE
  
  \STATE \textbf{Curriculum Scheduling:}
  \STATE Randomly partition $\mathcal{S}$ into $K$ groups.
  \STATE Sort $\mathcal{S}_i$ by reward $\bar{r}(x_i)$ (descending).
  \STATE Train $M$ incrementally on $\mathcal{S}_i$ from easy to hard.

  
  \STATE \textbf{Output:} Final ranked subset  $\mathcal{S}$.
  
  \end{algorithmic}
  \end{algorithm}



\subsection{Parameter Sensitivity Analysis}
\begin{figure}
    \centering
    \includegraphics[width=0.95\linewidth]{figures/para.pdf}
    \caption{Performance of Gemma-2-2b-it under different $\lambda$ values (subset size = 256).}
    \label{fig:para}
\end{figure}

The experiment examines the sensitivity of model performance to the regularization coefficient $\lambda$, which controls parameter regularization strength. Using the Gemma‑2‑2b‑it model with an embedding dimension of 256, $\lambda$ was varied over ${0.01, 0.1, 1, 10, 100, 1000}$, and performance was evaluated with NDCG@K and HR@K metrics ($K \in {5, 10, 20}$).

As shown in Fig.~\ref{fig:para}, performance improves as $\lambda$ increases from 0.01 to 1, peaking at $\lambda = 1$ (\textit{NDCG@5 = 0.0326}, \textit{HR@5 = 0.0476}). Moderate regularization thus mitigates overfitting and enhances generalization, whereas excessive regularization ($\lambda > 1$) constrains model learning. Consequently, $\lambda = 1$ is adopted as the default setting in subsequent experiments.
% The purpose of this experiment is to investigate the sensitivity of model performance to variations in the regularization coefficient $\lambda$, which controls the strength of parameter regularization. By systematically adjusting $\lambda$, we aim to understand its impact on the balance between model fitting and generalization.

% All experiments were conducted using the \textbf{Gemma-2-2b-it} model with the embedding dimension fixed at 256. The value of $\lambda$ was varied over the set $\{0.01, 0.1, 1, 10, 100, 1000\}$. For each setting, ranking performance was evaluated using two standard metrics: normalized discounted cumulative gain (\textbf{NDCG@K}) and hit ratio (\textbf{HR@K}), where $K \in \{5, 10, 20\}$. These metrics jointly measure the model’s ability to produce accurate and comprehensive ranked recommendations.

% As shown in Fig.~\ref{fig:para}, model performance is sensitive to the choice of $\lambda$. The results indicate that performance improves as $\lambda$ increases from 0.01 to 1, achieving the best overall results when $\lambda = 1$. Specifically, the model attains the highest scores across all evaluation metrics (\textit{NDCG@5 = 0.0326}, \textit{NDCG@10 = 0.0386}, \textit{NDCG@20 = 0.0445}, \textit{HR@5 = 0.0476}, \textit{HR@10 = 0.0662}, \textit{HR@20 = 0.0900}). This suggests that moderate regularization enhances generalization by mitigating overfitting. However, further increasing $\lambda$ beyond 1 leads to a gradual decline in performance, implying that excessive regularization restricts the model’s learning capacity.

% In summary, the optimal parameter setting for the \textbf{Gemma-2-2b-it} model is achieved at $\lambda = 1$, which provides the best trade-off between accuracy and generalization. Therefore, this value is adopted as the default in subsequent experiments.



==> sections/intro.tex <==
\section{Introduction}
The rapid advancement of large language models (LLMs) is propelling recommender systems into a new paradigm. 
Recent studies have shown that incorporating reinforcement learning (RL) into LLMs endows them with stronger \wl{reasoning and adaptablity} capabilities, 
thereby enabling a more accurate modeling of user preferences. 
% However, RL-based LLM recommendation faces critical challenges regarding data efficiency and training cost. 
% On the one hand, model performance is highly dependent on the quality of the data subsets used for RL optimization. 
% On the other hand, the computation of reward and advantage functions often requires multiple forward passes through the LLM. 
% \wl{However, RL-based LLM recommendation faces a critical challenge of data efficiency. 
% Model performance heavily depends on the quality and usefulness of the data subsets used for reinforcement learning, 
% and suboptimal sample selection can lead to unstable optimization and wasted computation.}
% For instance, optimization algorithms such as GRPO necessitate generating multiple trajectories per sample, 
% leading to substantial GPU memory consumption and training time. 
% This raises a key question: how can we efficiently select training data subsets while sustaining strong model performance in RL-based LLM recommendation?
\wl{However, RL-based LLM recommendation faces a critical challenge of data efficiency. 
Model performance heavily depends on the quality of data subsets used for reinforcement learning, 
and suboptimal sample selection can lead to unstable optimization. 
In particular, optimization algorithms such as GRPO require generating multiple trajectories for each sample, 
further amplifying the inefficiency and resulting in considerable computational overhead.}
This raises a key question: how can we effectively select training data subsets 
while sustaining strong model performance in RL-based LLM recommendation?

Data subset selection (or data pruning) seeks to reduce training cost while preserving, or even improving, model performance by identifying the most \wl{valuable} samples. 
Prior work in this area can be broadly grouped into three categories:
1. Signal-driven approaches: Selecting “hard” or “forgotten” samples based on gradient norms or loss signals.
2. Similarity/information-driven approaches: Enhancing diversity and coverage through clustering techniques or submodular optimization.
3. Meta-learning or active learning-driven approaches: Directly learning an optimal subset by employing bi-level optimization or meta-learned selection policies.
Despite notable progress, these approaches exhibit significant limitations in the context of RL-based LLM recommendation. Specifically: the sparsity and noise of reward signals undermine the reliability of signal-driven selection; 
similarity-based methods depend on embedding-space proximity, which poorly reflects semantic representativeness in text-driven RL tasks; 
learning-based approaches incur prohibitive computational cost on top of the already expensive RL optimization process.


Based on these insights, we identify two fundamental challenges for data pruning in RL-based LLM recommendation:
\begin{itemize}
    \item \textbf{Difficulty in measuring true optimization contribution.} 
    \wl{In GRPO-based training, optimization relies on \emph{relative} rewards (advantages) rather than absolute values. 
    Samples with high advantages can yield strong gradient signals even when their rewards stay consistently low. 
    These samples, which the model fails to learn effectively, still dominate updates due to misleading gradients. 
    Empirically, over one-quarter of samples (see Figure~\ref{fig:hit}) fall into this category, 
    showing that loss or gradient magnitude alone cannot reliably reflect true optimization value.}
    \item \textbf{Misalignment between embedding-space and \wl{optimization} representativeness.} 
    Existing methods typically assess representativeness in embedding space. 
    However, our k-means clustering experiments (see Table \ref{tab:kmeans}) 
    reveal that subsets selected by embedding representativeness perform even worse than random sampling. 
    \wl{This indicates that high embedding coverage does not translate to high training utility, 
    since embedding proximity does not necessarily imply similar gradient behavior or contribution to parameter updates.}
\end{itemize}




\begin{figure}[t]
    \centering
    \includegraphics[width=0.47\textwidth]{figures/hit_ratio_0_statistics.pdf}
    \caption{Comparison of hit ratio distributions before and after training. 
    Each horizontal bar shows the proportion of samples with zero hit ratio (red) and non-zero hit ratio (blue). 
    The shaded band highlights the subset of 557 samples (27.2\%) that 
    stayed at zero hit ratio both before and after training, 
    indicating that more than one quarter of the dataset consistently failed to achieve any hits throughout training.}
    \label{fig:hit}
\end{figure}

\begin{table}[t]
    \caption{Training results on \texttt{Gemma-2-2b-it} with 1,024 samples. 
    Random selection outperforms embedding-based K-means, 
    suggesting that embedding-space representativeness does not align with semantic training value. 
    Metrics: NDCG (N@k) and Hit Ratio (HR@k).}
    \label{tab:kmeans}
    \setlength{\tabcolsep}{3pt} 
    \begin{tabular}{ccccccc}
    \hline
    \multirow{2}{*}{method} & \multicolumn{6}{c}{CDs and Vinyl (1024)}              \\
                            & N@5 & N@10 & N@20 & HR@5   & HR@10  & HR@20  \\ \hline
    Random                  & 0.0297 & 0.0361  & 0.0419  & 0.0459 & 0.0657 & 0.0888 \\
    Kmeans                  & 0.0269 & 0.0349  & 0.0401  & 0.0445 & 0.0654 & 0.0875 \\ \hline
    \end{tabular}
\end{table}


% These challenges highlight the necessity of a new paradigm that can accurately estimate a sample's optimization value while ensuring semantic representativeness, 
% thereby enabling efficient yet effective pruning for RL-based LLM recommendation.

\wl{These challenges highlight the need for a new paradigm that can reliably estimate each sample's contribution to optimization,
thereby enabling efficient yet effective pruning for RL-based LLM recommendation.}


To address these challenges, we propose MiniRec, a data pruning framework tailored to RL-based LLM recommendation. 
The key idea of MiniRec is to construct a unified value function that integrates three dimensions—learnability, 
representativeness, and diversity—and iteratively selects the most valuable samples to form the training subset:
% 1. Learnability: Rather than relying solely on loss or gradient magnitude, MiniRec evaluates sample difficulty through reward-based learnability. 
% Trivially easy or excessively difficult samples contribute little, whereas samples of moderate difficulty provide the most informative optimization signals.
% 2. Representativeness: Instead of depending on embedding-space similarity, 
% MiniRec leverages gradient information to measure the alignment between a sample's gradient direction and the ideal optimization trajectory, 
% thereby ensuring that selected samples provide effective guidance for parameter optimization.
% 3. Diversity-enhanced unified value function: Considering only learnability and representativeness may still yield redundant selections. 
% To address this, MiniRec incorporates a Max-Min strategy to jointly model diversity. 
% Each candidate sample is assigned a dynamic marginal value that simultaneously accounts for 
% (i) optimization signal (learnability), (ii) trajectory alignment (representativeness), and (iii) marginal semantic coverage (diversity). 
% At each iteration, the sample with the highest overall value is chosen, ensuring a balanced subset that maximizes training utility.
\wl{\textbf{1. Learnability:}
To alleviate gradient noise from ineffective samples,
MiniRec replaces loss- or gradient-magnitude heuristics with a reward-based learnability metric. 
This criterion quantifies how much a sample can contribute to optimization given its reward learning potential: 
samples with extremely low and high rewards are down-weighted, while those of moderate rewards are prioritized 
for their informative and stable optimization signals.
\textbf{2. Representativeness:}
To address the misalignment between embedding-space and true optimization representativeness, 
MiniRec replaces embedding similarity with a gradient-based criterion that evaluates the alignment between each sample's gradient direction and the ideal optimization trajectory. 
This captures representativeness directly in optimization space, ensuring selected samples consistently contribute to effective parameter updates.
\textbf{(3) Diversity-enhanced unified value function.}
While learnability and representativeness ensure that selected samples are informative and optimization-relevant, 
considering only these two aspects may still lead to redundancy, as similar samples often convey overlapping optimization signals. 
To mitigate this, MiniRec incorporates a Max-Min strategy to explicitly encourage diversity in both semantic and optimization spaces. }

Each candidate sample is assigned a dynamic marginal value that combines learnability and representativeness under a diversity-aware weighting scheme.  
This unified score jointly accounts for a sample's optimization utility and its complementarity within the selected subset.  
At each iteration, MiniRec employs a Greedy Select strategy to choose the sample with the highest value, progressively forming a balanced and informative training set.

Beyond subset construction, MiniRec further employs curriculum learning to maximize utility. 
The selected subset is partitioned into batches, and training proceeds progressively from easier to harder samples. 
This curriculum schedule stabilizes early-stage optimization by preventing early exposure to overly difficult samples, 
while gradually exploiting the richer reward signals embedded in harder samples. With the unified value function, 
curriculum learning improves optimization stability and generalization.

Our contributions are three-fold:
\begin{itemize}
\item We systematically analyze the challenges of data pruning in RL-based LLM recommendation and propose principled metrics for evaluating sample value.
\item We develop MiniRec, which constructs a unified value function integrating learnability, representativeness, and diversity, 
    and further introduces curriculum learning to maximize efficiency.
\item Extensive experiments on multiple real-world recommendation datasets demonstrate that 
    MiniRec achieves comparable or superior performance with significantly reduced training cost compared to full-data training.
\end{itemize}

==> sections/method_backup.tex <==
\section{Methodology}

In this section, we present the key components of our proposed approach. 
We first introduce two criteria for evaluating the contribution of each sample to model training, namely \emph{learnability} and \emph{representativeness}. 
To further enhance the coverage of the selected data, we incorporate \emph{diversity} and formulate a dynamic unified value function that balances all three criteria. 
Based on this value function, an iterative selection strategy is employed to construct high-quality training subsets, which subsequently guide model optimization.


\begin{figure*}[t]
  \centering
  \includegraphics[width=0.8\textwidth]{figures/minirec.pdf}
  \caption{The MiniRec pipeline. 
  We estimate sample-level learnability, representativeness, and diversity 
  from the full training data, normalize these metrics, 
  and integrate them through a value function for greedy subset selection.
  The obtained subset $\mathcal{S}$ is then partitioned for 
  curriculum scheduling to train the model from easy to hard samples.}
  \label{fig:minirec}
\end{figure*}










% For clarity, we introduce the main symbols used throughout the MiniRec framework. 
% The full training dataset is denoted by $\mathcal{D}$, 
% and the candidate pool of not-yet-selected samples is $\mathcal{C}$. 
% The actively selected subset is written as $\mathcal{S}$. 
% Each sample is denoted by $x_i \in \mathcal{D}$, and its representation 
% (e.g., embedding or gradient-based feature) is $f(e_i)$. 
% The per-sample loss is $\ell(x_i; \theta)$ with respect to model parameters $\theta$, 
% and the gradient is $\nabla \ell(x_i)$. 
% These notations will serve as the foundation for later definitions of sample evaluation scores 
% and subset construction strategies.





\subsection{Reward-Based Learnability Estimation}

In reinforcement learning (RL)-based large language model (LLM) recommendation, 
the supervision signal is typically sparse and derived from \emph{relative} reward comparisons across multiple trajectories. 
As analyzed in the introduction, this property makes the conventional loss or gradient magnitude unreliable indicators of a sample’s true learnability. 
Samples that yield large gradients may still correspond to consistently low rewards, offering little optimization benefit, 
while those consistently achieving high rewards are trivially easy and contribute minimal new information. 
Hence, the most informative samples for optimization are those of \textit{moderate difficulty}—that is, moderately rewarded samples.

To operationalize this intuition, MiniRec defines a reward-based learnability score. 
For each training sample $x_i$, we obtain multiple rollout trajectories and corresponding reward signals. 
The mean reward over $N$ trajectories is computed as:
\begin{align}
\bar{r}(x_i) = \frac{1}{N}\sum_{n=1}^{N}r_n(x_i).
\end{align}
where $r_n(x_i)$ denotes the reward obtained from the $n$-th rollout of sample $x_i$, and $N$ is the total number of rollouts.
We then map the average reward into a continuous learnability score through a Gaussian-shaped function:
\begin{align}\label{eq:gaussian}
L(x_i) = \exp\!\left(-\frac{(\bar{r}(x_i) - \mu)^2}{2\sigma^2}\right),
\end{align}
where $\mu$ denotes the optimal “moderate difficulty” point (typically $\mu=0.5$) 
and $\sigma^2$ controls the tolerance around this target. 
This design ensures that both extremely easy (high-reward) and extremely hard (low-reward) samples are down-weighted, 
while samples with intermediate reward levels are prioritized as they carry the most valuable optimization signal.

A practical challenge arises in early-stage training: 
the model initially lacks meaningful recommendation ability, leading to most samples ($>90\%$) receiving rewards below $0.1$. 
In this regime, raw rewards are insufficiently discriminative to assess sample difficulty. 
To obtain a stable and cost-effective estimation, MiniRec adopts a two-stage reward approximation process:
\begin{enumerate}
  \item Randomly select a small subset (e.g., 256 samples) for a lightweight fine-tuning of the base model, constructing a proxy model that quickly calibrates the initial reward distribution.;
  \item Use the proxy to infer reward estimates $\bar{r}(x_i)$ for the entire dataset.
\end{enumerate}

Each estimated $\bar{r}(x_i)$ is then substituted into Eq.~\eqref{eq:gaussian} to obtain the provisional learnability score. 
To ensure comparability across samples and stable integration into the unified value function, 
we normalize the scores to $[0,1]$:
\begin{align}\label{eq:l_norm}
L_{\text{norm}}(x_i)=
\frac{L(x_i)-\min\limits_{x_j\in\mathcal{D}}L(x_j)}
{\max\limits_{x_j\in\mathcal{D}}L(x_j)-\min\limits_{x_j\in\mathcal{D}}L(x_j)}.
\end{align}

The normalized score $L_{\text{norm}}(x_i)$ serves as the final learnability score in MiniRec, 
quantifying how much each sample can potentially contribute to model optimization. 
By grounding learnability in reward-level information rather than loss or gradient magnitudes, 
this design directly aligns with RL training dynamics and mitigates the misleading effects of relative reward scaling.



\subsection{Gradient-Based Representativeness Estimation}

Beyond learnability, representativeness plays a crucial role in selecting effective training samples for RL-based LLM recommendation.  
While learnability reflects \emph{how much} a sample enables the model to learn, representativeness captures \emph{what direction} the model learns toward.  
Representative samples guide model updates along an optimization trajectory that better aligns with true reasoning learning, thereby accelerating convergence and enhancing stability.  

However, defining representativeness in this context is non-trivial.  
Traditional methods typically measure similarity or coverage in the embedding space, e.g., using clustering or submodular selection.  
Yet, as empirically verified in Table~\ref{tab:kmeans},  
embedding-space coverage does not guarantee optimization representativeness in RL-based recommendation.  
This is because RL training targets not only the mapping from $\textit{input}\!\rightarrow\!\textit{output}$,  
but also the intermediate reasoning process $\textit{input}\!\rightarrow\!\textit{reason}\!\rightarrow\!\textit{output}$.  
Embedding proximity may capture textual similarity but fails to reflect how each sample contributes to the \textit{reasoning optimization trajectory} of the model.

To address this misalignment, MiniRec defines representativeness directly in the \emph{optimization space} rather than the \emph{embedding space}.  
The key insight is that the optimization trajectory learned by reinforcement learning implicitly encodes the model’s reasoning dynamics— 
thus, samples whose gradients are more aligned with this trajectory are more representative for reasoning learning.

Formally, for each sample $x_i$, we compute its sample gradient
\begin{align}
v_i = \nabla_{h}\ell(x_i; \theta),
\end{align}
where $\ell(x_i; \theta)$ denotes the loss computed under model parameters $\theta$, and $h$ denotes the hidden state of the last token at the final layer for sample $x_i$.
The approximate global optimization direction can be defined as the mean gradient across all data:
\begin{align}\label{eq:g_first}
g = \frac{1}{|\mathcal{D}|}\sum_{x_i \in \mathcal{D}} v_i.
\end{align}

However, relying solely on first-order gradients can be unreliable in RL-based training,  
as early-stage gradients are often noisy due to unstable reward signals.  
To obtain a more faithful estimation of each sample’s optimization contribution,  
MiniRec incorporates second-order information through a {Hessian–Vector Product (HVP)} formulation.  
For each sample $x_i$, the HVP is defined as:
\begin{align}\label{eq:hvp}
\text{HVP}(x_i) = H(x_i) \cdot v_i 
= \nabla^2_{\theta}\ell(x_i; \theta)\, \nabla_{h}\ell(x_i; \theta),
\end{align}
where $H(x_i)$ is the Hessian of the loss with respect to $\theta$.  
This operation implicitly captures the local curvature of the optimization landscape along the gradient direction,  
offering a second-order refinement of a sample’s optimization influence—without explicitly forming the full Hessian matrix.

The refined global optimization trajectory is then approximated as:
\begin{align}\label{eq:g_star_hvp}
g^{(2)} = \frac{1}{|\mathcal{D}|}\sum_{x_i \in \mathcal{D}}\text{HVP}(x_i).
\end{align}

For each sample $x_i$, MiniRec defines its {representativeness score} as the cosine similarity between its HVP-adjusted gradient and the global second-order direction:
\begin{align}\label{eq:r}
R(x_i) = \cos\!\big( \text{HVP}(x_i),\, g^{(2)} \big).
\end{align}

Finally, the representativeness scores are normalized into $[0,1]$ following the scaling scheme in Eq.~\eqref{eq:l_norm}.  
A higher $R_{\text{norm}}(x_i)$ indicates stronger alignment with the ideal RL optimization direction,  
meaning the sample better encapsulates the reasoning-driven update trajectory.  
By leveraging this gradient-based alignment principle,  
MiniRec effectively selects samples that are truly representative for the reinforcement learning optimization process,  
rather than merely similar in embedding space.




\subsection{Sample Diversity}

While learnability and representativeness identify the most informative and directionally aligned samples, 
selecting solely based on them can lead to redundancy. 
Samples that are highly learnable and representative often cluster around similar optimization regions, 
resulting in subsets dominated by medium-difficulty samples with near-duplicate reasoning trajectories. 
This redundancy narrows the coverage of the optimization landscape, 
suppresses exposure to diverse reasoning patterns, and may cause overfitting or convergence stagnation.  
Therefore, a third core objective of MiniRec is to ensure diversity, 
which preserves heterogeneity in the training signals and enables the model to explore a broader reasoning space.

In contrast to learnability and representativeness—both intrinsic to individual samples—  
diversity is a \emph{relational property} defined with respect to the subset currently being constructed.  
It measures how distinct a candidate sample is from those already selected.  
Assigning a static diversity score independent of the selected set $\mathcal{S}$ would thus be inappropriate.  
To explicitly encourage non-redundant selection,  
MiniRec formulates diversity as a dynamic marginal value through a min–max strategy, 
enforcing maximal incremental diversity at each selection step.

Formally, let $f(x_i)$ denote the feature representation of sample $x_i$  
(e.g., the final-layer hidden state or task-specific embedding),  
and $\mathcal{S}$ be the currently selected subset.  
The marginal diversity contribution of a candidate $x_i$ is defined as its minimal distance to the subset:
\begin{align}
D(x_i \mid \mathcal{S}) = \min_{x_j \in \mathcal{S}} \,\mathrm{dist}\!\left(f(x_i), f(x_j)\right),
\end{align}
where $\mathrm{dist}(\cdot,\cdot)$ denotes the distance metric, which is instantiated as cosine distance in this paper.
This function yields high values for samples that lie far from the existing subset in the representation space, 
thus directly promoting sample differentiation.

To maintain consistency with other objectives,  
the diversity score is normalized to $[0,1]$, resulting in $D_{\text{norm}}(x_i \mid \mathcal{S})$.  
The overall selection value for a candidate $x_i$ is then defined as:
\begin{align}
V(x_i \mid \mathcal{S})
= D_{\text{norm}}\!\left(x_i \mid \mathcal{S}\right)
\Big[L_{\text{norm}}(x_i) + \lambda \, R_{\text{norm}}(x_i)\Big],
\end{align}
where $L_{\text{norm}}(x_i)$ and $R_{\text{norm}}(x_i)$ denote the normalized learnability 
and representativeness scores, respectively.  
The coefficient $\lambda$ balances the relative emphasis of optimization alignment versus reward sensitivity.

Subset construction proceeds iteratively with a greedy selection rule.  
At each step, the sample with the highest overall value is chosen:
\begin{align}
x^{*} = \arg\max_{x_i \in \mathcal{C}} V(x_i \mid \mathcal{S}),
\end{align}
and added to $\mathcal{S}$ as $\mathcal{S} \leftarrow \mathcal{S} \cup \{x^{*}\}$.  
This process continues until the target subset size is reached.  

The min–max design ensures that each newly selected sample maximizes marginal diversity 
while reinforcing learnability and representativeness.  
As a result, the constructed subset maintains broad coverage over the optimization space, 
preserves diverse reasoning trajectories, 
and achieves a balanced selection across learning difficulty, optimization alignment, 
and reasoning diversity—completing MiniRec’s tri-objective sample selection framework.





\subsection{Curriculum Scheduling}

While the selected subset $\mathcal{S}$ already encapsulates balanced learnability, representativeness, 
and diversity, directly training on $\mathcal{S}$ in a mixed and unordered manner may not yield 
optimal optimization dynamics.  
Samples of vastly different difficulty levels can interfere with each other, 
causing unstable gradient updates and suboptimal convergence, particularly in reasoning-intensive tasks.  

To address this, MiniRec introduces a {curriculum scheduling mechanism} 
that structures the learning process from easier to more challenging samples, 
thereby stabilizing optimization while maintaining diversity across stages.  
This design ensures that the model progressively internalizes foundational reasoning patterns 
before being exposed to harder, more heterogeneous cases.  

Concretely, the selected subset $\mathcal{S}$ is randomly partitioned into $K$ disjoint groups:
\begin{align}
\mathcal{S} = \mathcal{S}_1 \cup \mathcal{S}_2 \cup \cdots \cup \mathcal{S}_K, 
\quad \mathcal{S}_i \cap \mathcal{S}_j = \emptyset \;\; (i \neq j).
\end{align}
Within each partition $\mathcal{S}_i$, 
samples are further sorted in descending order of their reward values $r(x_i)$, 
ensuring internal progression from easier to more complex instances 
while keeping each group representative of the overall data distribution.  

The combination of random partitioning and intra-group ordering is crucial.  
If we globally sort the entire subset $\mathcal{S}$ by difficulty and train the model strictly from easy to hard, 
the training process would become too rigid.  
Because RL-based instruction tuning usually runs for only a few epochs, 
the model would focus heavily on the easiest samples at the beginning, 
quickly fitting their simple patterns and converging to a suboptimal solution.  
Once the model locks into these easy patterns, 
it becomes difficult for later, harder samples to effectively influence learning, 
which can even lead to a decline in performance.  

In contrast, MiniRec’s hybrid scheduling avoids this issue.  
Randomly partitioning the subset keeps each training phase diverse, 
while sorting within each group still provides a clear sense of progression from easier to harder cases.  
This design keeps the curriculum balanced—stable yet flexible—so the model avoids early overfitting, 
benefits from varied learning signals, 
and gradually strengthens its reasoning ability throughout training.



\begin{figure*}[htbp]
  \centering
  \includegraphics[width=0.75\textwidth]{figures/curriculum.pdf}
  \caption{Illustration of curriculum scheduling.}
  \label{fig:curriculum}
\end{figure*}



\begin{algorithm}[t]
  \caption{Subset Selection with Curriculum Scheduling}
  \label{alg:minirec}
  \begin{algorithmic}[1]
  
  \REQUIRE Full dataset $\mathcal{D}$, base model $M$, 
  target subset size $m$, balance weight $\lambda$, 
  number of curriculum groups $K$.
  
  \vspace{0.5em}
  \STATE \textbf{Learnability:} 
  Estimate rewards $\bar{r}(x_i)$, compute $L(x_i)$ (Eq.~\eqref{eq:gaussian}), 
  and normalize to $L_{\text{norm}}(x_i)$ (Eq.~\eqref{eq:l_norm}).
  
  \STATE \textbf{Representativeness:} 
  Compute representativeness score $R_{\text{norm}}(x_i)$ for each sample.
  
  \STATE \textbf{Diversity-driven Greedy Selection:}
  \STATE Initialize $\mathcal{S} \leftarrow \emptyset$.
  \WHILE{$|\mathcal{S}| <$ target size $m$}
    \FORALL{$x_i \in \mathcal{D} \setminus \mathcal{S}$}
      \STATE Compute diversity score $D_{\text{norm}}(x_i \mid \mathcal{S})$
             as minimum distance to samples in $\mathcal{S}$.
      \STATE Compute overall value:
        \[
        V(x_i \mid \mathcal{S}) = D_{\text{norm}}(x_i \mid \mathcal{S})
        \cdot \big( L_{\text{norm}}(x_i) + \lambda R(x_i) \big).
        \]
    \ENDFOR
    \STATE Select $x^* = \arg\max_{x_i} V(x_i \mid \mathcal{S})$.
    \STATE Update $\mathcal{S} \leftarrow \mathcal{S} \cup \{x^*\}$.
  \ENDWHILE
  
  \STATE \textbf{Curriculum Scheduling:}
  \STATE Randomly partition $\mathcal{S}$ into $K$ groups.
  \STATE Sort $\mathcal{S}_i$ by reward $\bar{r}(x_i)$ (descending).
  \STATE Train $M$ incrementally on $\mathcal{S}_i$ from easy to hard.

  
  \STATE \textbf{Output:} Final ranked subset  $\mathcal{S}$.
  
  \end{algorithmic}
  \end{algorithm}
